Ego4o: Egocentric Human Motion Capture and Understanding from Multi-Modal Input

This work focuses on tracking and understanding human motion using consumer wearable devices, such as VR/AR headsets, smart glasses, cellphones, and smartwatches. These devices provide diverse, multi-modal sensor inputs, including egocentric images, and 1-3 sparse IMU sensors in varied combinations. Motion descriptions can also accompany these signals. The diverse input modalities and their intermittent availability pose challenges for consistent motion capture and understanding. In this work, we present Ego4o (o for omni), a new framework for simultaneous human motion capture and understanding from multi-modal egocentric inputs. This method maintains performance with partial inputs while achieving better results when multiple modalities are combined. First, the IMU sensor inputs, the optional egocentric image, and text description of human motion are encoded into the latent space of a motion VQ-VAE. Next, the latent vectors are sent to the VQ-VAE decoder and optimized to track human motion. When motion descriptions are unavailable, the latent vectors can be input into a multi-modal LLM to generate human motion descriptions, which can further enhance motion capture accuracy. Quantitative and qualitative evaluations demonstrate the effectiveness of our method in predicting accurate human motion and high-quality motion descriptions.

==> sec/bak/0_abstract_bak_1.tex <==
\begin{abstract}
Tracking and understanding human motion in daily life is crucial for many applications, yet professional devices are inaccessible to most people, making it essential to leverage consumer-owned wearable devices like VR/AR headsets, smart glasses, cellphones, or smartwatches.
These devices offer diverse, multi-modal sensor inputs, with some modes appearing intermittently, posing challenges for human motion capture and understanding.
In this work, we present Ego4o (o for omni), a novel framework for simultaneous human motion capture and understanding from multi-modal inputs. The inputs may contain the arbitrary combination of egocentric images, 1-3 sparse IMU sensors, and human motion descriptions that can be obtained from wearable devices like VR/AR headsets, smartphones, earphones, and smartwatches.
First, the IMU sensor inputs, along with the optional egocentric image and text description of human motion, are encoded into the latent space of a pre-trained motion VQ-VAE. Next, the latent vectors are sent to the VQ-VAE decoder and optimized to track human motion. These latent vectors also serve as input to a fine-tuned multi-modal LLM to get the text description of human motion.
We also prove that the generated human motion description can be used to enhance the accuracy of the human motion capture.
Quantitative and qualitative evaluations demonstrate the effectiveness of our method in predicting accurate human motion and producing high-quality human motion descriptions from multi-modal input.
\end{abstract}

==> sec/bak/0_abstract_bak_2.tex <==
\begin{abstract}
This work focuses on tracking and understanding human motion using consumer wearable devices, such as VR/AR headsets, smart glasses, cellphones, and smartwatches. These devices provide diverse, multi-modal sensor inputs, including egocentric images, and 1-3 sparse IMU sensors in varied combinations. Motion descriptions can also accompany these signals.
% \DL{technically, those devices do not provide human motion description, so I would not write it here. We can write that motion description can accompany these signals (without specifying how they are obtained)}
%
The diverse input modalities and their intermittent availability pose challenges for consistent motion capture and understanding. In this work, we present \textit{Ego4o} (\textit{o} for omni), a new framework for simultaneous human motion capture and understanding from multi-modal inputs.
%
\DL{
First, the IMU sensor inputs, along with the optional egocentric image and text description of human motion, are encoded into the latent space of a pre-trained motion VQ-VAE. Next, the latent vectors are sent to the VQ-VAE decoder and optimized to track human motion. When motion descriptions are unavailable, the latent vectors can be input into a fine-tuned multi-modal LLM to generate human motion descriptions, which can further enhance motion capture accuracy.
-- I would rephrase this part a bit to highlight what is really unique in this method: multi-modal and optional inputs. After reading this, the reader should be able to understand in a high level what is the main technical contribution that makes it possible.
}
%
Quantitative and qualitative evaluations demonstrate the effectiveness of our method in predicting accurate human motion and producing high-quality human motion descriptions from multi-modal input.
\vspace{-1em}
\end{abstract}

==> sec/bak/1_intro_bak_1.tex <==
\section{Introduction}
\label{sec:intro}
Accurate tracking and understanding of human motion are essential for applications in healthcare, sports, rehabilitation, VR/AR, and human-computer interaction. While professional systems like motion capture suits and multi-view studios deliver accurate results, they are costly and inaccessible to most users. Recent methods using single third-view RGB cameras offer an alternative but are either constrained to fixed spaces or require a dynamic camera held by another person/device, limiting their practicality.
This underscores the need for human motion capture and understanding solutions that utilize the widely available wearable devices like VR/AR headsets, smart glasses, cellphones, and smartwatches. 
These devices provide diverse, multi-modal sensor inputs related to human motion, such as inertial measurement unit (IMU) data, egocentric camera images, and potentially even voice-enabled conversation data. 

While these on-body devices provide a wealth of data modalities, existing works only focus on motion capture from one single modality. Some methods~\cite{luo2021dynamics, li2023ego, wang2024egocentric} predict the human motion from the stream of egocentric cameras, while some other methods capture the human motion from VR tracker~\cite{jiang2022avatarposer, castillo2023bodiffusion} or IMU signals~\cite{mollyn2023imuposer, yi2022physical}. 
Each individual modality provides only a limited view of human motion, constraining the accuracy of both motion capture and understanding. For example, the full human body motion is barely seen or significantly occluded from the egocentric camera. 
Text descriptions can offer information about human motion categories but lack the precision to detail specific movements. 
IMUs on VR/AR headsets, smartwatches, and cellphones are very sparse: they usually only track the movement of one or two limbs, as people rarely wear watches on both wrists. 

We observe that different input modalities serve complementary roles in motion analysis. Motion descriptions and egocentric images provide rich semantic context about both the activity being performed and the environmental setting. For example, when the egocentric view shows a desk in close proximity, it strongly indicates that the person is in a seated position. Simultaneously, IMU signals from wearable devices capture precise kinematic data for specific body segments. For instance, a smartwatch's IMU sensors can capture detailed hand movements, enabling the system to differentiate between blocking and smashing motions in table tennis, which may be indiscernible from the egocentric camera perspective alone.
\RD{Although it reads good, we should not spend three paragraphs to justify the setting. I would suggest we squeeze it into two. sometimes, a good use-case figure can also be used to help convey these points.}
\par

However, leveraging multi-modalities from wearable devices is not straightforward, since the input availability can change over time. The egocentric camera and microphone might be disabled for privacy reasons. The number and location of IMUs are also variable, as users may remove a phone from their pocket or increase their IMU count by wearing a smartwatch. \RD{this sounds like a repeat of the paragraph 2.}

To address these challenges and to fully leverage the information from wearable devices, we introduce Ego4o, a novel framework designed to capture and understand human motion using multi-modal data from everyday wearable devices. 
%
Ego4o utilizes 1–3 sparse IMU sensors, along with optional egocentric images and motion descriptions, to accurately capture 3D human motion. Additionally, it can simultaneously generate human motion descriptions.
% , enhancing both motion capture and interpretive capabilities.
\RD{Noteably, we show that the internal motion tokenization can also be used to generate descriptions of the human motion and facilitate motion related conversations with a Large Language Model.
%
What's more, we show that using the in-context reasoning and image understanding capabilities of a Large Language Model can allow us to provide textual descriptions that lead to better motion recovery. Rephrase.}

We begin by training a multimodal transformer to encode various inputs into motion tokens using a part-based Vector Quantized Variational Autoencoder (VQ-VAE). To ensure flexibility in handling different combinations of multimodal inputs, we implement random masking of IMU sensor data, egocentric images, and motion descriptions during the training phase. These encoded motion tokens are subsequently processed by the VQ-VAE decoder to generate predictions of human motion. Additionally, we enhance the accuracy of these predictions through optimization in the VQ-VAE's latent space, leveraging the conditioning provided by IMU sensor data.


The motion tokens and egocentric images are then processed by a multi-modal large language model (LLM), which has been fine-tuned on multi-modal inputs to generate detailed textual descriptions of the captured movements. While obtaining accurate descriptions of human motion is typically challenging in real-world scenarios—which can limit the motion capture module's effectiveness—our work demonstrates that these LLM-generated textual descriptions can serve as valuable supplementary input to improve the overall accuracy of human motion capture.

We validate Ego4o's effectiveness through comprehensive quantitative and qualitative evaluations. Experimental results demonstrate that our proposed method achieves better motion capture accuracy on both the DIP-IMU~\cite{huang2018deep} and Nymeria~\cite{ma2024nymeria} datasets, while simultaneously generating detailed and accurate descriptions of human movements from multi-modal inputs—as validated on the Nymeria dataset~\cite{ma2024nymeria}. By integrating motion capture and motion understanding within a unified framework, Ego4o marks an advancement toward making motion analysis both accessible and practical for everyday applications through consumer devices.

\noindent In summary, our key contributions are the following:

\begin{itemize}
    \item We present Ego4o, a novel framework for egocentric human motion capture and understanding that flexibly accommodates various combinations of multi-modal inputs;
    \item The Ego4o framework seamlessly integrates kinematic data from sparse 1-3 IMU sensors with semantic context derived from egocentric images and textual descriptions, leveraging complementary modalities to achieve better motion capture and understanding;
    \item We demonstrate that AI-generated motion descriptions can improve the accuracy of egocentric human motion capture;
    \item We demonstrate the outstanding performance of this framework in both egocentric motion tracking and understanding tasks. 
\end{itemize}


% Our observation is that these different input modalities can complement each other. For example, the motion description and egocentric images can provide rich semantic context about human motion, like what the person is doing, and where the person is located. From the semantic motion context, the human motion can be roughly inferred. For example, a close-to-desk view indicates that the person is sitting. On the other hand, the IMU signals from body-worn devices can provide accurate kinematic information about a particular body part, such as hand movements. For example, sparse motion sensors can differentiate between the block and smash in table tennis, where these motions may appear identical in the egocentric view.

% Despite multiple input modalities can be provided, several challenges persist. 
% First, the input data can only provide limited information about the human body motion. Images captured by egocentric cameras usually cannot fully capture the human body. Text descriptions can offer information about the category of human motion but lack the precision to detail specific movements. IMUs on VR/AR headsets, smartwatches, and cellphones are very sparse: they usually only track the movement of one or two limbs—people generally do not wear watches on both wrists. 
% Furthermore, the number and the location of the IMUs are also uncertain and even change on the go: some people put their cell phones in the left pocket while others put them in the right pocket; some people can take out a phone from their pocket, or they can add to the number of IMUs by wearing their smartwatches.

% First, we propose a masked multi-modal transformer to encode the IMU sensor and optional image features into the token space of a part-based VQ-VAE. The tokens are further sent to the VQ-VAE decoder, where they are optimized to track human motion. Additionally, these vectors are used as input for a fine-tuned, multi-modal language model (LLM), which generates text-based descriptions of the captured motion from the motion token input and egocentric image input. Finally, by incorporating these textual descriptions into the motion-tracking process, we further enhance the performance and interpretability of the captured human motion.

% The effectiveness of Ego4o is demonstrated through quantitative and qualitative evaluations. Our experiments show that the proposed method achieves highly accurate motion capture results on both the DIP-IMU dataset~\cite{huang2018deep} and Nymeria dataset~\cite{ma2024nymeria}, while also generating meaningful and descriptive human motion descriptions from multi-modal inputs, which is evaluated on the Nymeria dataset~\cite{ma2024nymeria}. By enabling both motion capture and understanding in a single framework, Ego4o represents a step forward in making sophisticated motion analysis more accessible and practical for everyday use through consumer devices.



==> sec/bak/1_intro_bak_2.tex <==
\section{Introduction}
\label{sec:intro}
% Accurate tracking and understanding of human motion are essential for many applications. While professional systems deliver accurate results, they are costly and inaccessible to most users. 
% This underscores the need for human motion capture and understanding solutions that utilize widely available wearable devices like VR/AR headsets, smart glasses, cellphones, and smartwatches. 
Recently, more and more researches focus on human motion capture and understanding using widely available wearable devices like VR/AR headsets, smart glasses, cellphones, and smartwatches.
These devices provide diverse, multi-modal sensor inputs related to human motion, such as inertial measurement unit (IMU) data, egocentric camera images, and potentially even voice-enabled conversation data. 
However, existing works only focus on motion capture from one single input modality. Some methods~\cite{luo2021dynamics, li2023ego, wang2024egocentric} predict the human motion from egocentric cameras, while some other methods capture the human motion from VR tracker~\cite{jiang2022avatarposer, castillo2023bodiffusion} or IMU signals~\cite{mollyn2023imuposer, yi2022physical}. 
% While these on-body devices provide a wealth of data modalities, existing works only focus on motion capture from one single input modality. Some methods~\cite{luo2021dynamics, li2023ego, wang2024egocentric} predict the human motion from egocentric cameras, while some other methods capture the human motion from VR tracker~\cite{jiang2022avatarposer, castillo2023bodiffusion} or IMU signals~\cite{mollyn2023imuposer, yi2022physical}. 
Each individual modality provides only a limited view of human motion, constraining the accuracy of both motion capture and understanding. For example, the full human body motion is barely seen or significantly occluded from the egocentric camera. 
Text descriptions can offer information about human motion categories but lack the precision to detail specific movements. 
IMUs on VR/AR headsets, smartwatches, and cellphones are very sparse: they usually only track the movement of one or two limbs, as people rarely wear watches on both wrists. 

We observe that different input modalities serve complementary roles in motion analysis. Motion descriptions and egocentric images provide rich semantic context about both the activity being performed and the environmental setting. For example, when the egocentric view shows a desk in close proximity, it strongly indicates that the person is sitting. IMU signals from wearable devices capture precise kinematic data for specific body segments. For instance, a smartwatch's IMU sensors can capture detailed hand movements, enabling the system to differentiate between blocking and smashing motions in table tennis, which may be indiscernible from the egocentric camera perspective alone. 
% \JW{Maybe add a usecase figure?}

However, leveraging multi-modalities from wearable devices is not straightforward, since the input availability can change over time. The egocentric camera and microphone might be disabled. The number and location of IMUs are also variable over time, as users may remove a phone from their pocket or increase their IMU count by wearing a smartwatch. 
% \RD{this sounds like a repeat of the paragraph 2.}
To address these challenges and to fully leverage the information from wearable devices, we introduce \textbf{Ego4o} (o for omni), a novel framework designed to capture and understand human motion using multi-modal data from everyday wearable devices. The Ego4o examples are shown in \cref{fig:teaser}.
Ego4o utilizes 1–3 sparse IMU sensors, along with optional egocentric images and motion descriptions, to accurately capture 3D human motion. Additionally, it can simultaneously generate human motion descriptions.
Notably, we show that motion tokenization can be used to generate descriptions of human motion and facilitate motion-related conversations with a Large Language Model. Furthermore, we demonstrate that leveraging the in-context reasoning and image-understanding capabilities of a Large Language Model can enable us to provide textual descriptions that lead to improved motion capture.
% Noteably, we show that the motion tokenization can also be used to generate descriptions of human motion and facilitate motion-related conversations with a Large Language Model.
% What's more, we show that using the in-context reasoning and image understanding capabilities of a Large Language Model can allow us to provide textual descriptions that lead to better motion capture.

We begin by training a multi-modal transformer to encode various inputs into motion tokens using a part-based Vector Quantized Variational Autoencoder (VQ-VAE). To ensure flexibility in handling different combinations of multimodal inputs, we implement random masking of IMU sensor data, egocentric images, and motion descriptions during the training phase. These encoded motion tokens are subsequently processed by the VQ-VAE decoder to generate predictions of human motion. Additionally, we enhance the accuracy of these predictions through optimization in the VQ-VAE's latent space, leveraging the conditioning provided by IMU sensor data.


The motion tokens and egocentric images are then processed by a multi-modal large language model (LLM), which has been fine-tuned on multi-modal inputs to generate detailed textual descriptions of the captured movements. While obtaining accurate descriptions of human motion is typically challenging in real-world scenarios—which can limit the motion capture module's effectiveness—our work demonstrates that these LLM-generated textual descriptions can serve as valuable supplementary input to improve the overall accuracy of human motion capture.

We validate Ego4o's effectiveness through comprehensive quantitative and qualitative evaluations. Experimental results demonstrate that our proposed method achieves better motion capture accuracy on both the DIP-IMU~\cite{huang2018deep} and Nymeria~\cite{ma2024nymeria} datasets, while simultaneously generating detailed and accurate descriptions of human movements from multi-modal inputs—as validated on the Nymeria dataset~\cite{ma2024nymeria}. By integrating motion capture and motion understanding within a unified framework, Ego4o marks an advancement toward making motion analysis both accessible and practical for everyday applications through consumer devices.
\noindent In summary, our contributions are:

\begin{itemize}
    \item We present Ego4o, a novel framework for egocentric human motion capture and understanding that flexibly accommodates various combinations of multi-modal inputs;
    \item The Ego4o framework seamlessly integrates kinematic data from sparse 1-3 IMU sensors with semantic context derived from egocentric images and textual descriptions, leveraging complementary modalities to achieve better motion capture and understanding;
    \item We show that AI-generated motion descriptions can improve the accuracy of egocentric human motion capture;
    \item We demonstrate the outstanding performance of this framework in both egocentric motion tracking and understanding tasks.
\end{itemize}


% Our observation is that these different input modalities can complement each other. For example, the motion description and egocentric images can provide rich semantic context about human motion, like what the person is doing, and where the person is located. From the semantic motion context, the human motion can be roughly inferred. For example, a close-to-desk view indicates that the person is sitting. On the other hand, the IMU signals from body-worn devices can provide accurate kinematic information about a particular body part, such as hand movements. For example, sparse motion sensors can differentiate between the block and smash in table tennis, where these motions may appear identical in the egocentric view.

% Despite multiple input modalities can be provided, several challenges persist. 
% First, the input data can only provide limited information about the human body motion. Images captured by egocentric cameras usually cannot fully capture the human body. Text descriptions can offer information about the category of human motion but lack the precision to detail specific movements. IMUs on VR/AR headsets, smartwatches, and cellphones are very sparse: they usually only track the movement of one or two limbs—people generally do not wear watches on both wrists. 
% Furthermore, the number and the location of the IMUs are also uncertain and even change on the go: some people put their cell phones in the left pocket while others put them in the right pocket; some people can take out a phone from their pocket, or they can add to the number of IMUs by wearing their smartwatches.

% First, we propose a masked multi-modal transformer to encode the IMU sensor and optional image features into the token space of a part-based VQ-VAE. The tokens are further sent to the VQ-VAE decoder, where they are optimized to track human motion. Additionally, these vectors are used as input for a fine-tuned, multi-modal language model (LLM), which generates text-based descriptions of the captured motion from the motion token input and egocentric image input. Finally, by incorporating these textual descriptions into the motion-tracking process, we further enhance the performance and interpretability of the captured human motion.

% The effectiveness of Ego4o is demonstrated through quantitative and qualitative evaluations. Our experiments show that the proposed method achieves highly accurate motion capture results on both the DIP-IMU dataset~\cite{huang2018deep} and Nymeria dataset~\cite{ma2024nymeria}, while also generating meaningful and descriptive human motion descriptions from multi-modal inputs, which is evaluated on the Nymeria dataset~\cite{ma2024nymeria}. By enabling both motion capture and understanding in a single framework, Ego4o represents a step forward in making sophisticated motion analysis more accessible and practical for everyday use through consumer devices.



==> sec/bak/3_method_bak_1.tex <==
\section{Method}
In this section, we propose a novel method for simultaneous human motion capture and understanding using multi-modal inputs.
Our system processes a combination of egocentric images, textual motion descriptions, and data from one, two, or three IMU sensors. These IMU sensors can be positioned on the head, wrists, or legs—locations that correspond to the common placement of wearable devices such as VR headsets, smartwatches, and cellphones.
An overview of our approach is shown in Fig.~\ref{fig:framework}. 
In the following sections, we first discuss the training of part-based motion VQ-VAE (\cref{method:vqvae}), then introduce the approaches for multi-modal human motion capture (\cref{method:mocap}) and motion understanding (\cref{method:motion_understanding}).
We also show how the generated motion description can be used to further enhance the performance of motion capture module (\cref{method:gen_text}). \JW{add location of IMUs in introduction and here.}

\subsection{Learning Part-Aware Motion Representation}~\label{method:vqvae}

Learning discrete human motion representations with VQ-VAE~\cite{van2017neural} has proven effective in many human motion-related tasks, including human motion generation~\cite{guo2022tm2t, zhang2023generating} and motion-focused large language models~\cite{jiang2023motiongpt, chen2024motionllm, zhou2024avatargpt}. These works treat the human body as a holistic entity, encoding the full human body motion into a single VQ-VAE codebook. Even though this holistic encoding strategy is effective for many applications, it presents limitations for our specific use case. \RD{There are works that do non-holistic, part-wise splitting of the codebooks. Such as Bailando++. Also Anindita for her VAE (not VQVAE)}

Our method aims to support flexible IMU sensor configurations, ranging from a single head-mounted IMU in smart glasses to various combinations of sensors embedded in smartwatches and smartphones. To achieve this adaptability, we implement the part-aware VQ-VAE architecture introduced in TLControl~\cite{wan2023tlcontrol}, which establishes separate motion codebooks for individual body segments.
These separate motion codebooks enable the direct projection of available IMU signals into their corresponding part-specific motion codebooks, while simultaneously facilitating the generation of latent features for body segments lacking sensor coverage. 
For example, when processing data from a wrist-mounted IMU, the system not only projects this information into the arm-specific motion codebook but also generates leg movements.
% For example, when processing data from a wrist-mounted IMU, the system not only projects this information into the arm-specific motion codebook but also generates motion features for other body segments—such as leg movements—by conditioning on the available wrist sensor data.
This projection mechanism operates analogously to a text-infilling task~\cite{lewis2019bart}, where the system infers motion patterns for unmonitored body segments based on the available sensor data. By employing this part-aware architecture, our system achieves better motion capture accuracy across diverse IMU configurations, offering a more versatile solution compared to conventional holistic approaches. 


% Our method supports arbitrary IMU sensor layout: sometimes only the IMU on the smart glasses (head) is provided, and sometimes the IMU on the left wrist (smartwatch) and right thigh(cellphone) is provided. Considering this, we propose to learn separate human motion codebook for each human body part with the part-aware VQ-VAE proposed in TLControl~\cite{wan2023tlcontrol}, and then project the IMU signals to their corresponding motion latent space. For example, the IMU data from the right wrist will be projected into the motion codebook of the right arm. This process can be seen as a text-in-filling task~\cite{lewis2019bart}: the motion code corresponding to unavailable IMUs will be generated from other available IMUs. With this strategy, we can enhance the performance of motion capture from arbitrary IMU layouts.

In the following paragraphs, we detail how to learn the motion representation with part-aware VQ-VAE.
Specifically, all the joints are first divided into six joint groups, including Head, Left arm, Right arm, root, Left leg, and Right leg. The input ground truth human motion is first encoded to the HumanML3D~\cite{guo2022generating} representation $J\in \mathbb{R}^{T\times M}$, where $T$ is the motion length and the $M=263$ corresponds to the dimensions of the overparameterized human motion representation. Next, this HumanML3D representation in each time step is split into six groups according to the correlated human body part: $J = [J_{Head}, J_{LArm}, J_{RArm}, J_{LLeg}, J_{RLeg}, J_{Root}]$. \RD{The subscript text should be under the $\text{Root}$ tag.}
%
For each body part $i$, \RD{we train a separate}\sout{there is a unique} encoder $\mathcal{E}_i$ to learn an independent codebook $C_i\in \mathbb{R}^{N_\text{code} \times d}$, where $N_\text{code}$ is the size of codebook while $d$ is the dimension of each codebook. The encoder first encodes the human motion into features $Q_i \in \mathbb{R}^{T' \times d}$, where $T' = T/4$. 
%
Next, the $Q_i$ is quantized with $C_i$, obtaining the quantized feature $\hat{Q}_i$. The quantized features from all of the body parts are finally concatenated and sent to the VQ-VAE decoder $\mathcal{D}$ to get the reconstructed full body motion $\hat{J}_\text{recon}$.
\RD{We don't need to overload the notations with a hat, if you're never going to use $Q_i$ again.}

For training the part-aware VQ-VAE, we use standard loss terms including quantization, commitment, and reconstruction losses:

\begin{equation}
\begin{aligned}
    \mathcal{L} = \sum_{i} & \left( \beta \| \text{sg}[\hat{Q}_i] - Q_i \|_2 \right. \\
& + \left. \| \hat{Q}_i - \text{sg}(Q_i) \|_2 \right)  + \| J - \hat{J}_\text{recon} \|_2
\end{aligned}
\end{equation}
where $\beta$ is a balancing term, $\text{sg}[\cdot]$ denotes the stop-gradient operator.

Having established a part-aware discrete representation of human motion, we proceed to project multi-modal features into this representational space, utilizing it for both motion capture and motion understanding tasks. \JW{Shrink this part}

\subsection{Multi-Modal Human Motion Capture}~\label{method:mocap}

In this section, we introduce our multi-modal human motion capture method. The process begins with a transformer-based multi-modal encoder that projects IMU signals, egocentric images, and motion descriptions into the motion representation space learned by the VQ-VAE. These motion features are then processed by the VQ-VAE decoder to reconstruct human motion. Additionally, we offer an optional test-time optimization procedure that can further enhance the accuracy of the motion capture results.

\subsubsection{Multi-Modal Encoder}


Our transformer-based multi-modal encoder processes three input types: motion description $T_m$, egocentric images $I$, and IMU signal sequences \RD{No symbol for IMUs? :-)}. 
%
The egocentric image $I$ and motion description $T_m$ are encoded into image features $F_I$ and textual features $F_T$ respectively using CLIP~\cite{radford2021learning}. The IMU signal sequence comprises acceleration vectors $A \in \mathbb{R}^{T\times N_{imu} \times 3}$ and rotation matrices $R \in \mathbb{R}^{T\times N_{imu} \times 3 \times 3}$, where $T$ represents the sequence length and $N_{imu} = 5$ denotes the total number of possible IMU sensors. \RD{Should we mention that $N_{\text{imu}}$ is the \textit{maximum} number of IMUs that we work with. In practice, our method is designed to works with arbitrary number of IMUs.}
%
The rotation matrices $R$ are converted to 6D representations~\cite{zhou2019continuity} $R_{6d} \in \mathbb{R}^{T\times N_{imu} \times 6}$.
The IMU acceleration and rotation data are then concatenated and reshaped into an input IMU sequence $F_{imu}$ of length $T'N_{imu}$\RD{What is $T'$?}. 
%
These IMU sequences $F_{imu}$, along with the image features $F_I$ and the textual motion description features $F_T$, are processed through an embedding layer before being fed into a transformer encoder~\cite{vaswani2023attentionneed}. 
%
The encoder predicts the logits of the motion code IDs $L_{t, i}$ for the $i^{th}$ IMU at each time step $t$ of the input sequence. Finally, we employ Gumbel Softmax~\cite{jang2016categorical} to get the motion code index $\text{Ind}_i \in \{0, 1, 2, ..., N_\text{code}\}$ of the corresponding $i^{th}$ IMU and select the quantized motion feature $\hat{Q}_{t, i}$ from the motion code book. \RD{Should we use $\delta_i$ for the index? Or is $\text{Ind}_i$ common?}
%
The quantized motion features are sent to the VQ-VAE decoder $\mathcal{D}$ following the same way in \cref{method:vqvae} to get the human motion prediction $\hat{J}$. The multi-modal encoder can be trained with the following loss function, which includes the motion code classification loss and human motion reconstruction loss:

\begin{equation}
    \mathcal{L} = \mathbb{E}_{\hat{L} \sim P(L)} \left( -\log P(\hat{L} | A, R, I, T_m) \right) + \left\| \hat{J} - J \right\|_2
\end{equation}

To simulate real-world scenarios where certain input modalities may be unavailable, we implement a masking strategy during training. This involves randomly masking egocentric images and textual descriptions. We also simultaneously select random combinations of one to three IMU sensors as active inputs. The remaining IMU sensors are masked to ensure our model learns to operate effectively with varying levels of sensor availability.

% Our transformer-based multi-modal encoder takes the motion description $T_{motion}$, egocentric images $I$, and a sequence of IMU signals as input. The egocentric image $I$ and the motion description $T_{motion}$ are encoded to image features $F_I$ and $F_T$ with Clip~\cite{radford2021learning}. The sequence of the IMU signal contains the IMU acceleration vector $A \in \mathbb{R}^{T\times N_{imu} \times 3}$ and IMU rotation matrix $R \in \mathbb{R}^{T\times N_{imu} \times 3 \time 3}$, where the $T$ is the length of the input sequence, $N_{imu} = 5$ is the number of all possible IMUs. The IMU rotation matrix $R$ is converted to the 6d representation~\cite{zhou2019continuity} $R_{6d} \in \mathbb{R}^{T\times N_{imu} \times 6}$. 
% Then, the IMU acceleration and rotation are concatenated and reshaped to the input IMU sequence $F_{imu}$ with length $T' \times N_{imu}$. The input IMU sequence $F_{imu}$, image features $F_I$ and motion description features $F_T$ are further processed with the embedding layer and finally sent to the transformer encoder~\cite{vaswani2023attentionneed} to predict the motion features $Q_{t, i}$ for the $i$th IMU at time step $t$ of the input sequence. Finally, we use the motion codebook of the $i$th limb $C_i$ in \cref{method:vqvae} to quantize the predicted motion feature $Q_{t, i}$ of the corresponding $i$th IMU, obtaining the quantized motion feature $\hat{Q}_{t, i}$ and code index $\text{Ind} \in {0, 1, 2, ..., N_\text{code}}$.



\subsubsection{Test-Time Optimization} \label{method:optim}

After obtaining the human motion prediction $\hat{J}$, we can further refine the accuracy of our motion capture through an optional test-time optimization procedure.
The task of the optimization process is to find a motion feature $Q$ in the VQ-VAE latent space such that the reconstructed human motion $J = \mathcal{D}(Q)$ minimizes the following objective
function:

\begin{equation}
    E(J) = \lambda_a E_a(J, A) + \lambda_r E_r (J, \textbf{R})
\end{equation}

where $E_a(\cdot)$, $E_r(\cdot)$ are the IMU acceleration term and IMU orientation term respectively, which we will describe in detail later. \RD{I only see two terms, a = accleration, r = rotation. Where is the smoothness term?}
%
In our experiment, we set the weights $\lambda_a = 0.01$, $\lambda_r = 0.1$, $\lambda_t = 1$, respectively. We use smaller weights for the IMU accelerations since they are more noisy. \RD{These are implementation details. Better not to break flow of the text by specifying them immediately.}

For simplicity, we assume IMUs are positioned near their corresponding body joints—for instance, a smartphone's IMU approximates hip joint motion.
To compute the IMU acceleration term, we first calculate the acceleration of each joint position that corresponds to an IMU sensor placement. For the joint associated with the $i$th\RD{$i^{th}
$} IMU at time step $t$, the acceleration is calculated using: $\hat{a}^i_t = (J^i_{t+2} - 2J^i_{t+1} + J^i_t)/(\Delta t^2)$, where $\Delta t = 1$ in our experiment. 

The overall IMU acceleration term is calculated as: $E_a(J, A) =\sum_i\sum_t\| \hat{a}^i_t - a^i_t \|_2$, where $t = 0, 1, 2, ...$ represents time steps in the motion sequence, $i$ indexes the available IMU sensors.

To compute the IMU orientation term, we first calculate the orientation of each limb in predicted motion $\hat{J}$ that corresponds to an IMU sensor placement. For the limb associated with the $i$th IMU at time step $t$, the orientation vector is calculated using: $\hat{r}^i_t = (J^i_{t, \text{child}} - J^i_{t, \text{parent}}) / \|J^i_{t, \text{child}} - J^i_{t, \text{parent}}\|_2$
where $J^i_{t, \text{child}}$ and $J^i_{t, \text{parent}}$ represent the child and parent joint positions of the limb segment associated with the $i$th IMU.

Next, we calculate the ground truth orientation of each available IMU sensor with $r^i_t = \textbf{M}^i \cdot \textbf{R}^i_t \cdot [0, 1, 0]^T$
where $\textbf{R}^i_t$ represents the rotation matrix of the $i$th IMU at time step $t$, $[0, 1, 0]^T$ denotes the initial orientation vector, and $\textbf{M}^i$ represents the calibration rotation matrix between the IMU sensor and its corresponding limb segment, determined through prior calibration. The IMU orientation term is then computed as:
$E_r(J, R) = \sum_i\sum_t\|\hat{r}^i_t - r^i_t\|_2$, where $i$ indexes the available IMU sensors.

\RD{I feel this section is too long. We have had almost 2 pages of text on just how to tokenize the motion.}
\subsection{Egocentric Human Motion Understanding}~\label{method:motion_understanding}

In this section, we present our approach to human motion understanding through multi-modal LLM fine-tuning. While existing pre-trained multi-modal LLMs excel at modeling language and image distributions, they lack the capability to process data related to human motion. To address this limitation, we extend LLaVA~\cite{liu2024visual} by incorporating a new motion modality and fine-tuning it using the multi-modal egocentric dataset Nymeria~\cite{ma2024nymeria}. 
% Finally, we discuss that the generated text description can further enhance the motion capture qualtiy.

\subsubsection{Architecture}

\begin{figure}
\centering
\includegraphics[width=1\linewidth]{fig/LLM/LLM_crop.pdf}
\caption{
Egocentric Human Motion Understanding Architecture. 
\vspace{-2em}
}
\label{fig:llm}
\end{figure}

The architecture of our egocentric LLM is shown in \cref{fig:llm}.
Given an input image $I$ and IMU sensor data $(A, R)$, we first employ the multi-modal encoder described in \cref{method:mocap} to generate human motion codes, which serve as discrete motion tokens. These motion codes are then processed through a linear embedding layer $\mathbf{E}_M$ to produce human motion features $H_M$, aligned with the language model's word embedding dimensionality. Since we assume text descriptions are unavailable during motion description generation, we exclude them from the multi-modal encoder input.
For image processing, we utilize a pretrained Clip~\cite{radford2021learning} image encoder $\mathbf{E}_I$ to map image features $F_I$ into the word embedding space, resulting in $H_I$. 
Finally, the image features $H_I$, motion features $H_M$, and text encodings $H_T$ are concatenated and fed into the large language model to generate the response.

\subsubsection{Training}

For each IMU signal sequence $(A, R)$ and corresponding egocentric image $I$, we generate conversation pairs $(X_q, X_a)$. The questions $X_q$ are randomly sampled prompts requesting human motion descriptions, while the answers $X_a$ are drawn from the fine-grained motion descriptions in the Nymeria~\cite{ma2024nymeria} dataset. The input instruction is constructed as $X_\text{ins} = \text{Random Select} \{ [I, X_q], [A, R, X_q], [A, R, I, X_q] \}$.

The LLM can be fine-tuned on prediction tokens using an auto-regressive training objective. The probability of generating the answer $X_a$ is computed as:
\begin{equation}
p(X_a | X_\text{ins}) = \prod_{i=1}^{L} p_{\theta}(x_i | X_v, X_{\text{ins}, <i}, X_{a, <i})
\end{equation}
where $L$ represents the token sequence length, $\theta$ denotes the trainable parameters, and $X_{\text{ins},<i}$ and $X_{a,<i}$ are the instruction and answer tokens preceding the current prediction token $x_i$. The trainable parameters are optimized using the negative log-likelihood loss.

The training process consists of two stages: in the first stage, we conduct motion pre-training to achieve motion feature alignment. In the second stage, we use multi-modal fine-tuning to enable egocentric motion understanding. 

\textbf{Motion Pre-Training.}
For the pre-training phase, we restrict input instructions to those containing only IMU signals $[A, R, X_q]$. To ensure proper alignment between motion features and the pre-trained LLM's word embeddings, we exclusively train the motion embedding layer $\mathbf{E}_M$ while keeping all other architectural components frozen.

\textbf{Multi-Modal Finetuning.}
During this training phase, we maintain frozen weights for both the CLIP encoder and multi-modal encoder, while continuing to update three components: the image embedding layer $\textbf{E}_I$, motion embedding layer $\textbf{E}_M$, and LLM parameters with LoRA~\cite{hu2021lora}.

\subsection{Generated Description for Better MoCap}\label{method:gen_text}

While our motion capture module functions effectively without verbal descriptions, incorporating high-quality motion descriptions can significantly enhance its accuracy. However, obtaining such descriptions in real-world scenarios presents a challenge, as users are typically reluctant to narrate their actions in real time. To address this limitation, we leverage our system's ability to generate accurate motion descriptions through the Ego4o LLM. Although these generated descriptions may not perfectly match human-provided ground truth descriptions, they prove valuable for enhancing motion capture performance. To further bridge the gap between generated and ground truth descriptions, we fine-tuned our multi-modal encoder using these generated descriptions for only 300 iterations, with results detailed in our ablation study (\cref{exp:ablation}).

==> sec/bak/3_method_bak_2.tex <==
\section{Method}
% In this section, we propose a novel method (Fig.~\ref{fig:framework}) for simultaneous human motion capture and understanding using multi-modal inputs.
Our method (Fig.~\ref{fig:framework}) processes a combination of egocentric images $I$, textual motion descriptions $X_a$, and data from one, two, or three IMU sensors, including device acceleration $A$ and rotation $R$. The IMU sensors may be placed at up to five locations: the head, wrists, or hips, reflecting typical placements for devices like VR headsets, smartwatches, and cellphones. From these multi-modal inputs, we achieve accurate motion capture and can generate motion descriptions when they are absent.
To achieve this, we first train a part-based motion VQ-VAE (\cref{method:vqvae}) to learn the discrete motion representation, then use the multi-modal encoder to project the inputs to the motion representation space(\cref{method:mocap}). The discrete motion codes can also be used for generating motion descriptions (\cref{method:motion_understanding}).
Finally, we show the generated motion description can be used to enhance the performance of the motion capture (\cref{method:gen_text}). 
% An overview of our approach is shown in Fig.~\ref{fig:framework}. 

\subsection{Learning Part-Aware Motion Representation}~\label{method:vqvae}

In this section, we learn discrete human motion representation with VQ-VAE~\cite{van2017neural} and further enable the projection of multi-modal inputs to the motion representation space. 
% Learning discrete human motion representations with VQ-VAE~\cite{van2017neural} has proven effective in many human motion-related tasks, including human motion generation~\cite{guo2022tm2t, zhang2023generating} and motion-focused large language models~\cite{jiang2023motiongpt, chen2024motionllm, zhou2024avatargpt}. 
Most previous works~\cite{guo2022tm2t, zhang2023generating, jiang2023motiongpt, chen2024motionllm, zhou2024avatargpt} treat the human body as a holistic entity, encoding the full human body motion into a single VQ-VAE codebook. Though this holistic encoding is effective, it presents limitations for our use case. 
% \RD{There are works that do non-holistic, part-wise splitting of the codebooks. Such as Bailando++. Also Anindita for her VAE (not VQVAE)}

Our method aims to support flexible IMU sensor configurations, ranging from a single head-mounted IMU in smart glasses to various combinations of sensors embedded in smartwatches and smartphones. To achieve this adaptability, we implement the part-aware VQ-VAE architecture introduced in TLControl~\cite{wan2023tlcontrol}, which establishes separate motion codebooks for individual body segments.
These separate motion codebooks enable the direct projection of available IMU signals into their corresponding part-specific motion codebooks, while simultaneously facilitating the generation of latent features for body segments lacking sensor coverage. 
For example, when processing data from a wrist-mounted IMU, the system not only projects this information into the arm-specific motion codebook but also generates leg movements.
% For example, when processing data from a wrist-mounted IMU, the system not only projects this information into the arm-specific motion codebook but also generates motion features for other body segments—such as leg movements—by conditioning on the available wrist sensor data.
This projection mechanism operates analogously to a text-infilling task~\cite{lewis2019bart}, where the system infers motion patterns for unmonitored body segments based on the available sensor data. By employing this part-aware architecture, our system achieves better motion capture accuracy across diverse IMU configurations, offering a versatile solution compared to conventional holistic approaches. 


% Our method supports arbitrary IMU sensor layout: sometimes only the IMU on the smart glasses (head) is provided, and sometimes the IMU on the left wrist (smartwatch) and right thigh(cellphone) is provided. Considering this, we propose to learn separate human motion codebook for each human body part with the part-aware VQ-VAE proposed in TLControl~\cite{wan2023tlcontrol}, and then project the IMU signals to their corresponding motion latent space. For example, the IMU data from the right wrist will be projected into the motion codebook of the right arm. This process can be seen as a text-in-filling task~\cite{lewis2019bart}: the motion code corresponding to unavailable IMUs will be generated from other available IMUs. With this strategy, we can enhance the performance of motion capture from arbitrary IMU layouts.

Next, we discuss how to learn the motion representation with part-aware VQ-VAE.
Specifically, all the joints are first divided into six joint groups, including head, left arm, right arm, root, left leg, and right leg. The input ground truth human motion is first encoded to the HumanML3D~\cite{guo2022generating} representation $J\in \mathbb{R}^{T\times M}$, where $T$ is the motion length and $M=263$ corresponds to the HumanML3D dimensions \DL{instead of using HumanML3D representation/dimensions, can we use a more generic name and refer to \cite{guo2022generating}? maybe human motion representation?}. Next, $J$ in each time step is split into six groups according to the correlated human body part: $J = [J_\text{Head}, J_\text{LArm}, J_\text{RArm}, J_\text{LLeg}, J_\text{RLeg}, J_\text{Root}]$.
%
For each body part $i$, we train a separate encoder $\mathcal{E}_i$ to learn an independent codebook $C_i\in \mathbb{R}^{N_\text{code} \times d}$, where $N_\text{code}$ is the size of codebook while $d$ is the dimension of each codebook. The encoder first encodes the human motion into features $Q_i \in \mathbb{R}^{T' \times d}$, where $T' = T/4$. 
%
Next, the $Q_i$ is quantized with $C_i$ \DL{that means quantized based on the obtained code book? it is not very clear}, obtaining the quantized feature $\hat{Q}_i$. The quantized features from all of the body parts are finally concatenated and sent to the VQ-VAE decoder $\mathcal{D}$ to get the reconstructed full body motion $\hat{J}_\text{recon}$.
% For training the part-aware VQ-VAE, we use standard loss terms including quantization, commitment, and reconstruction losses. The details are shown in the suppl. mat.
The training of the part-aware VQ-VAE is detailed in the suppl. mat.
Next, we project multi-modal features into this representational space for motion capture and motion understanding. \DL{can we elaborate more on this? Or if this is explained in another subsection, we can refer to it here, otherwise is seems that details are missing.}

\subsection{Multi-Modal Human Motion Capture}~\label{method:mocap}

In this section, we introduce our multi-modal human motion capture method. The process begins with a transformer-based multi-modal encoder that projects IMU signals, egocentric images, and motion descriptions into the motion representation space learned by the VQ-VAE. These motion features are then processed by the VQ-VAE decoder to reconstruct human motion. Additionally, we offer an optional test-time optimization procedure that can further enhance the accuracy of the motion capture results.

\subsubsection{Multi-Modal Encoder}


Our transformer-based multi-modal encoder processes three input types: motion description $T_m$, egocentric images $I$, and IMU signal sequences. 
%
The egocentric image $I$ and motion description $T_m$ are encoded into image features $F_I$ and textual features $F_T$ respectively using CLIP~\cite{radford2021learning}. The IMU signal sequence comprises acceleration vectors $A \in \mathbb{R}^{T\times N_{imu} \times 3}$ and rotation matrices $R \in \mathbb{R}^{T\times N_{imu} \times 3 \times 3}$, where $T$ represents the sequence length and $N_{imu} = 5$ is the \textit{maximum} number of IMU locations. In practice, our method is designed to work with arbitrary number of IMUs. 
% \RD{Should we mention that $N_{\text{imu}}$ is the \textit{maximum} number of IMUs that we work with. In practice, our method is designed to works with arbitrary number of IMUs.}
%
The rotation matrices $R$ are converted to 6D representations~\cite{zhou2019continuity} $R_{6d} \in \mathbb{R}^{T\times N_{imu} \times 6}$.
The IMU acceleration and rotation data are then concatenated and reshaped into an input IMU sequence $F_{imu}$ of length $T'\times N_{imu}$, where $T' = T/4$. 
%
These IMU sequences $F_{imu}$, along with the image features $F_I$ and the textual motion description features $F_T$, are processed through an embedding layer before being fed into a transformer encoder~\cite{vaswani2023attentionneed}. 
%
The encoder predicts the logits of the motion code IDs $L_{t, i}$ for the $i^{th}$ IMU at each time step $t$ of the input sequence. Finally, we employ Gumbel Softmax~\cite{jang2016categorical} to get the motion code index $\delta_i \in \{0, 1, 2, ..., N_\text{code}\}$ of the corresponding $i^{th}$ IMU and select the quantized motion feature $\hat{Q}_{t, i}$ from the motion code book. 
%
The quantized motion features are sent to the VQ-VAE decoder $\mathcal{D}$ following the same way in \cref{method:vqvae} to get the human motion prediction $\hat{J}$. The multi-modal encoder can be trained with the following loss function, which includes the motion code classification loss and human motion reconstruction loss:

\begin{equation}
    \mathcal{L} = \mathbb{E}_{\hat{L}} \left( -\log P(\hat{L} | A, R, I, T_m) \right) + \lambda \left\| \hat{J} - J \right\|_2
\end{equation}
where $\lambda$ is the weight of reconstruction loss.
To simulate real-world scenarios where certain input modalities may be unavailable, we implement a masking strategy during training. This involves randomly masking egocentric images and textual descriptions. We also simultaneously select random combinations of one to three IMU sensors as active inputs. The remaining IMU sensors are masked to ensure our model learns to operate effectively with varying sensor availability.


\subsubsection{Test-Time Optimization} \label{method:optim}

Limb movement in the motion prediction $\hat{J}$ may not fully align with the corresponding IMU's acceleration and orientation. This can be refined through optional test-time optimization.
% After obtaining the human motion prediction $\hat{J}$, we can further refine the accuracy of our motion capture through an optional test-time optimization.
The task is to find a motion feature $Q$ in the VQ-VAE latent space such that the reconstructed human motion $J = \mathcal{D}(Q)$ minimizes the energy
function:

\begin{equation}
    Q = \argmin_Q \lambda_a E_a(J, A) + \lambda_r E_r (J, \textbf{R})
\end{equation}

where $E_a(\cdot)$, $E_r(\cdot)$ are the IMU acceleration term and IMU orientation term respectively.
For simplicity, we assume IMUs are positioned near their corresponding body joints—for instance, a smartphone's IMU approximates hip joint motion.
To compute the IMU acceleration term, we first calculate the acceleration of each joint position that corresponds to an IMU sensor placement. For the joint associated with the $i^{th}$ IMU at time step $t$, the acceleration is calculated using: $\hat{a}^i_t = (J^i_{t+2} - 2J^i_{t+1} + J^i_t)/(\Delta t^2)$, where $\Delta t = 1$ in our experiment. 
%
The overall IMU acceleration term is calculated as: $E_a(J, A) =\sum_i\sum_t\| \hat{a}^i_t - a^i_t \|_2$, where $t = 0, 1, 2, ...$ represents time steps in the motion sequence, $i$ indexes the available IMU sensors.

To compute the IMU orientation term, we first calculate the orientation of each limb in predicted motion $\hat{J}$ that corresponds to an IMU sensor placement. For the limb associated with the $i$th IMU at time step $t$, the orientation vector is calculated using: $\hat{r}^i_t = (J^i_{t, \text{child}} - J^i_{t, \text{parent}}) / \|J^i_{t, \text{child}} - J^i_{t, \text{parent}}\|_2$
where $J^i_{t, \text{child}}$ and $J^i_{t, \text{parent}}$ represent the child and parent joint positions of the limb segment associated with the $i$th IMU.

Next, we calculate the orientation of each available IMU sensor with $r^i_t = \textbf{M}^i \cdot \textbf{R}^i_t \cdot [0, 1, 0]^T$
where $\textbf{R}^i_t$ represents the rotation matrix of the $i$th IMU at time step $t$, $[0, 1, 0]^T$ denotes the initial orientation vector, and $\textbf{M}^i$ represents the calibration rotation matrix between the IMU sensor and its corresponding limb segment, determined through prior calibration. The IMU orientation term is then computed as:
$E_r(J, R) = \sum_i\sum_t\|\hat{r}^i_t - r^i_t\|_2$, where $i$ indexes the available IMU sensors.

\subsection{Egocentric Human Motion Understanding}~\label{method:motion_understanding}

In this section, we present our approach to human motion understanding through multi-modal LLM fine-tuning. While existing pre-trained multi-modal LLMs excel at modeling language and image distributions, they lack the capability to process data related to human motion. To address this limitation, we extend LLaVA~\cite{liu2024visual} by incorporating a new motion modality and fine-tuning it using the multi-modal egocentric dataset Nymeria~\cite{ma2024nymeria}. 
% Finally, we discuss that the generated text description can further enhance the motion capture qualtiy.

\subsubsection{Architecture}

\begin{figure}
\centering
\includegraphics[width=1\linewidth]{fig/LLM/LLM_crop.pdf}
\caption{
Egocentric Human Motion Understanding. Each modality is encoded separately and then concatenated in the order specified by the input instruction $X_\text{ins}$ before being fed into the LLM.
\vspace{-1em}
}
\label{fig:llm}
\end{figure}

The architecture of our egocentric LLM is shown in \cref{fig:llm}.
Given an input image $I$ and IMU sensor data $(A, R)$, we first employ the multi-modal encoder described in \cref{method:mocap} to generate human motion codes, which serve as discrete motion tokens. These motion codes are then processed through a linear embedding layer $\mathbf{E}_M$ to produce human motion features $H_M$, aligned with the language model's word embedding dimensionality. Since we assume text descriptions are unavailable during motion description generation, we exclude them from the multi-modal encoder input.
For image processing, we utilize a pretrained Clip~\cite{radford2021learning} image encoder $\mathbf{E}_I$ to map image features $F_I$ into the word embedding space, resulting in $H_I$. 
Finally, the image features $H_I$, motion features $H_M$, and text encodings $H_T$ are concatenated and fed into the LLM to generate the response.

\subsubsection{Training}

For each IMU signal sequence $(A, R)$ and corresponding egocentric image $I$, we generate conversation pairs $(X_q, X_a)$. The questions $X_q$ (see an example in \cref{fig:llm}) are randomly sampled prompts requesting human motion descriptions, while the answers $X_a$ are drawn from the fine-grained motion descriptions in the Nymeria~\cite{ma2024nymeria} dataset. The input instruction is constructed as $X_\text{ins} = \text{Random Select} \{ [I, X_q], [A, R, X_q], [A, R, I, X_q] \}$.

The LLM can be fine-tuned on prediction tokens using an auto-regressive training objective. The probability of generating the answer $X_a$ is computed as:
\begin{equation}
p(X_a | X_\text{ins}) = \prod_{i=1}^{L} p_{\theta}(x_i | X_v, X_{\text{ins}, <i}, X_{a, <i})
\end{equation}
where $L$ represents the token sequence length, $\theta$ denotes the trainable parameters, and $X_{\text{ins},<i}$ and $X_{a,<i}$ are the instruction and answer tokens preceding the current prediction token $x_i$. The trainable parameters are optimized using the negative log-likelihood loss.

The training process consists of two stages: in the first stage, we conduct motion pre-training to achieve motion feature alignment. In the second stage, we use multi-modal fine-tuning to enable egocentric motion understanding. 

\textbf{Motion Pre-Training.}
For the pre-training phase, we restrict input instructions to those containing only IMU signals $[A, R, X_q]$. To ensure proper alignment between motion features and the pre-trained LLM's word embeddings, we exclusively train the motion embedding layer $\mathbf{E}_M$ while keeping all other architectural components frozen.

\textbf{Multi-Modal Finetuning.}
During this training phase, we maintain frozen weights for both the CLIP encoder and multi-modal encoder, while continuing to update three components: the image embedding layer $\textbf{E}_I$, motion embedding layer $\textbf{E}_M$, and LLM parameters with LoRA~\cite{hu2021lora}.

\subsection{Generated Description for Better MoCap}\label{method:gen_text}

While our motion capture module functions effectively without verbal descriptions, incorporating high-quality motion descriptions can significantly enhance its accuracy. However, obtaining such descriptions in real-world scenarios presents a challenge, as users are typically reluctant to narrate their actions in real time. To address this limitation, we leverage our system's ability to generate accurate motion descriptions through the Ego4o LLM. Although these generated descriptions may not perfectly match human-provided reference descriptions, they prove valuable for enhancing motion capture performance. To further bridge the gap between generated and ground truth descriptions, we fine-tuned our multi-modal encoder using these generated descriptions for only 300 iterations, with results detailed in our ablation study (\cref{exp:ablation}).
